Photometry as a proxy for stellar activity in radial velocity analyses

Stellar activity remains a limiting factor in measuring precise planet parameters from radial velocity spectroscopy, not least in the search for Earth mass planets orbiting in the habitable zones of Sun-like stars. One approach to mitigate stellar activity is to use combined analyses of both radial velocity and time-series photometry. We present an analysis of simultaneous disk-integrated photometry and radial velocity data of the Sun in order to determine the useful limits of a combined analysis. We find that simple periodogram or autocorrelation analysis of solar photometry give the correct rotation period <50% of the time. We therefore use a Gaussian process to investigate the time variability of solar photometry and to directly compare simultaneous photometry with radial velocity data. We find that the hyperparameter posteriors are relatively stable over 70 years of solar photometry and the amplitude tracks the solar cycle. We observe good agreement between the hyperparameter posteriors for the simultaneous photometry and radial velocity data. Our primary conclusion is a recommendation to include an additional prior in Gaussian process fits to constrain the evolutionary timescale to be greater than the recurrence timescale (ie., the rotation period) to recover more physically plausible and useful results. Our results indicate that such simultaneous monitoring may be a useful tool in enhancing the precision of radial velocity surveys.

==> main <==
\BOOKMARK [1][-]{section*.1}{ABSTRACT}{section*.2}% 1
\BOOKMARK [1][-]{section.1}{Introduction}{}% 2
\BOOKMARK [1][-]{section.2}{Solar Datasets}{}% 3
\BOOKMARK [2][-]{subsection.2.1}{Initial Data Comparisons}{section.2}% 4
\BOOKMARK [2][-]{subsection.2.2}{EMPIRE Data Periodicities}{section.2}% 5
\BOOKMARK [1][-]{section.3}{Methods}{}% 6
\BOOKMARK [2][-]{subsection.3.1}{Introduction to Gaussian Processes}{section.3}% 7
\BOOKMARK [2][-]{subsection.3.2}{Fitting a Gaussian Process}{section.3}% 8
\BOOKMARK [1][-]{section.4}{Results}{}% 9
\BOOKMARK [2][-]{subsection.4.1}{Solar Temporal Variations using EMPIRE}{section.4}% 10
\BOOKMARK [2][-]{subsection.4.2}{Direct Comparison of Photometry with Radial Velocity Data}{section.4}% 11
\BOOKMARK [1][-]{section.5}{Conclusion}{}% 12

